Prefix tuning for automated audio captioning

Audio captioning aims to generate text descriptions from environmental sounds. One challenge of audio captioning is the difficulty of the generalization due to the lack of audio-text paired training data. In this work, we propose a simple yet effective method of dealing with small-scaled datasets by leveraging a pre-trained language model. We keep the language model frozen to maintain the expressivity for text generation, and we only learn to extract global and temporal features from the input audio. To bridge a modality gap between the audio features and the language model, we employ mapping networks that translate audio features to the continuous vectors the language model can understand, called prefixes. We evaluate our proposed method on the Clotho and AudioCaps dataset and show our method outperforms prior arts in diverse experimental settings.

==> Sections/1_related_works.tex <==
The audio captioning task is firstly introduced by Drossos~\etal~\cite{drossos2017automated}, which designed GRU-based encoder-decoder architecture. Following the primary work, most of the prior arts approached this task with encoder-decoder structure~\cite{}, where the encoder is trained from and decoder trained     


The first research of Automated Audio Captioning(AAC) was proposed by Drossos et al.\cite{drossos2017automated}. The method made by Drossos et al. has an encoder-decoder structure that composed of GRU-based encoder and decoder. Most of the models for AAC usually have an encoder-decoder structure\cite{mei2021audio}\cite{xu2021investigating}, where the encoder is trained from pre-trained weights and the decoder is trained from scratch. Many method determine to use RNN or LSTM as decoder for creating caption, recently transformer layer-based networks are often used. But, these networks are easy to cause overfitting when using small-scale dataset\cite{xue2021bayesian}, which may property of almost datasets in AAC due to the cost of collecting audio and annotated captions. The methods of using large-scale language model in AAC were proposed a few times. Especially, Koizumi et al.\cite{koizumi2020audio} proposed a method that uses GPT2 in the process of creating a caption, and it is most similar to our method. But this method uses GPT2 for giving an information of retrieved captions, therefore limits the capabilities of a large-scale language model. We will, however, approach to AAC task by using prefix tuning\cite{li2021prefix} that can exploit the expressiveness and generalization ability of the language model.
